Towards Split Learning-based Privacy-Preserving Record Linkage

Split Learning has been recently introduced to facilitate applications where user data privacy is a requirement. However, it has not been thoroughly studied in the context of Privacy-Preserving Record Linkage, a problem in which the same real-world entity should be identified among databases from different dataholders, but without disclosing any additional information. In this paper, we investigate the potentials of Split Learning for Privacy-Preserving Record Matching, by introducing a novel training method through the utilization of Reference Sets, which are publicly available data corpora, showcasing minimal matching impact against a traditional centralized SVM-based technique.

==> sections/previous_versions/evaluation_00.tex <==

%%%%%%

\begin{figure*}[t!]
\begin{minipage}[b]{0.47\textwidth}
         \includegraphics[width=\columnwidth]{media/reference_size_Precision.eps}
          % \vspace{-0.15in}
        \subcaption{\footnotesize{Precision vs. method vs. RS size.}}
        \label{fig:reference_size_Precision}
    \end{minipage}
    % \hfill        
    \begin{minipage}[b]{0.47\textwidth}
        \includegraphics[width=\columnwidth]{media/reference_size_Recall.eps}
          % \vspace{-0.15in}
        \subcaption{\footnotesize{Recall vs. method vs. RS size.}}
        \label{fig:reference_size_Recall}
    \end{minipage}
    \begin{minipage}[b]{0.47\textwidth}
            \includegraphics[width=\columnwidth]{media/train_size_Precision.eps}
          % \vspace{-0.15in}
        \subcaption{\footnotesize{Precision vs. method vs. training size.}}
        \label{fig:training_size_Precision}
    \end{minipage}
    % \hfill
    % \vspace{0.1in}
    \begin{minipage}[b]{0.47\textwidth}
        \includegraphics[width=\columnwidth]{media/train_size_Recall.eps}
          % \vspace{-0.15in}
        \subcaption{\footnotesize{Recall vs. method vs. training size.}}
        \label{fig:training_size_Recall}
    \end{minipage}
    % \hfill
     \caption{Results of the Experimental Evaluation.}
    \label{fig:experiments}
\end{figure*}\section{Empirical Evaluation}
\label{sec:evaluation}
To evaluate the performance of our method, we conducted a series of experiments and measured matching quality and execution time. In this section, we present our results, but first we will describe the data sets we have used and our experimental setup.

\subsection{Experimental Setup and Datasets}
For our evaluation we have used Python 3, and scikit-learn\footnote{Implementation available at: \url{https://github.com/mikez3/Split-Learning-Privacy-Preserving-Record-Linkage}}. We ran our experiments on a Core i5-10600K host with 16GB of main memory powered by Ubuntu 22.04. 

We used recordsets coming from the North Carolina voters database\footnote{\url{https://dl.ncsbe.gov/?prefix=data}}, having used three samples with 2000, 5000 records and 10000 records each. In each sample, we have used the following string attributes: ‘last name’, ‘first name’ and ‘middle name’ and deduplicated the dataset so that these attributes form a candidate key. Then, we generated two databases. The first one belongs to Alice, while the second one belongs to Bob. Since we are interested in linking low quality data, we corrupted Bob’s records using the German Record Linkage Center’s data corrupter \cite{Corrupter}, with the dataset on Bob's side containing one error per row for the corrupted records, so that a join operation using these quasi-identifiers yields an empty result set. As our method features a Reference Set, we created two reference sets, one with 200 records and one with 2000 records using actor names from Wikipedia\footnote{\url{https://en.wikipedia.org/w/index.php?title=Category:20th-century_American_male_actors}}. These were built so that no attribute value from the recordsets is found in the Reference Sets.

%%%%%%

We measure matching performance, in terms of correctly matched record pairs using Precision and Recall. Precision is defined as the fraction of the relevant elements among the retrieved elements, while Recall is defined as the fraction of the retrieved relevant elements divided by the total relevant elements: $Precision = \frac{{TP}}{TP + FP}$ and $Recall = \frac{{TP}}{TP + FN}$. At this point, we have to stress that each party performs matching individually. As such, matching performance varies, depending on the performance of the SVM model trained locally. To this end, we report Precision and Recall separately so as to provide a more detailed view of our method's performance. We also report time efficiency in terms of testing time.

To have a broader view of our method, we considered two setups for our SVM classifier. The first setup employs a linear SVM kernel with a hyperparameter C=100 at both parties, while the second one employs an RBF kernel with C=0.01 at both parties. We have used Edit Distance as a distance function between the Reference Set and each party's recordset and Cosine Distance to calculate the distances between the resulting distance vectors. For each setup, we have performed three executions and report the average results for Precision, Recall and matching time. Finally, to be able to have a basis of comparison, we also compare against a single local SVM classifier, as described in \cite{christen2008automatic}.

\subsection{Evaluation of Matching Performance}
To evaluate the matching performance and the behavior of our method, we will consider the size of the reference set used and the size of the training set used. We will vary these parameters and examine how our method behaves with respect to the dataset sample size used for matching in terms of Precision and Recall. 

\paragraph{Impact of Reference Set Size} Let us begin our assessment by varying the Reference Set size, while using a training dataset equal to 2000 records. The results of this set of experiments are illustrated in Fig. \ref{fig:reference_size_Precision} and \ref{fig:reference_size_Recall}. The horizontal axis represents the size of the dataset we attempted to match, while the vertical axis the respective measure, i.e. Precision or Recall. We report results both for the linear and RBF kernels. For the results of the Split process, we illustrate results for both reference set sizes for each of the matching, designated by `-1-' for Alice and `-2-' for Bob, while the case of simple SVM, without privacy characteristics is designated by ``Plain''.

We will first present our Precision results (Fig. \ref{fig:reference_size_Precision}) starting with the Plain SVM training, with Precision values of above 0.98 and in the area of 0.97. We can see that, in this case, Precision is not affected by dataset size. Next, for the case of split learning, first of all, we can see that, in all cases, precision deteriorates as the size of the matching dataset increases. Furthermore, the size of the Reference Set does not seem to affect performance. What affects matching performance is the type of the classifier to be used. As such, RBF kernels seem to have, in most cases, slightly better performance compared to the performance of linear kernels. Furthermore, there are slight fluctuations in precision between Alice and Bob, something which is anticipated, since each of them has been trained using different data. 

Let us discuss now Recall performance, as illustrated in Fig. \ref{fig:reference_size_Recall}. First, we may discern that both Plain SVM classifiers achieve absolute Recall, without being affected by matching set sizes. The performance of the Split Learning classifiers has not been deteriorated, in this case, as opposed to the case of Precision, when the size of the matching dataset increases. In this case, there is a drop in performance by 1.3\% when linear kernels have been used and less than 2\% when RBF kernels are used. For both parties the performance is aligned. On the other hand, the size of the Reference Set used does not incur any impact. 



%Starting with Precision, we can discern that the highest precision is for the Local Linear SVM with a values above 0.98. Then the RBF SVM follows with a performance in the area of 0.97. We may observe that these classifiers are not affected by the dataset sizes to be matched. Then, we proceed to the Federated classifiers. Our first observation is that the Linear classifier's performance is superior than all other cases in terms of Precision, for both dataset sizes. Also, using Reference Sets of different sizes does not seem to affect performance. Nevertheless, in this case, Precision is affected by the size of the datasets to be matched. Even in these cases the difference from the Local Liner classifier is in the area of 0.01, which is the cost to be paid to achieve privacy-preserving characteristics. On the other hand, as in the Local case, neither RBF kernels seem to behave towards the desired direction. Using a smaller Reference Set, the RBF kernel lacks up to 0.05 compared to the Local RBF kernel for the 10000 records dataset and approximately 0.06 from the Local Linear kernel. However, when increasing the size of the Reference Set, the situation significantly improves and this difference halves to 0.02 and 0.03 respectively.

%Examining, now, Recall, as illustrated in Fig. \ref{fig:reference_size_Recall}, we first observe that both Local SVM classifiers achieve perfect Recall, without being affected by matching set sizes. The Linear Federated classifier is not affected by dataset size either, nor by the size of the Reference Set used. Nevertheless, it performs lower than the Local classifiers by 5\%. The RBF kernels, again, come last. However, in this case their performance is not affected by the dataset size they are used at. On the contrary, their performance is affected by the Reference Set size used to train them. As such, the RBF's Recall vastly improves from 0.85 to 0.9 when increasing the size of the Reference Set.

\paragraph{Impact of Training Set Size} Now, to examine the impact of the Training set size on matching performance, we change our setup keeping the Reference Set size fixed to 2000 records, while we vary the size of the Training set. Particularly, we consider two training setups, one with 500 records and one with 2000 records. The results of this part of our evaluation for Precision and Recall are illustrated in Fig. \ref{fig:training_size_Precision} and Fig. \ref{fig:training_size_Recall} respectively. These Figures have been setup in a similar way with  Fig. \ref{fig:reference_size_Precision} and Fig. \ref{fig:reference_size_Recall}, so we will move ahead and describe the results. 

We will begin again with Precision and consider the case of Plain SVMs. For the Linear SVM, Precision reached 0.98, regardless of the Training Set size and it is not affected by the size of the dataset to be matched. The Plain RBF SVM comes second in terms of performance when trained with the 2000 records dataset, with Precision between near 0.975, while when it is trained with the smaller Training dataset, its precision drops slightly below 0.94. 

Now, when it comes to the outcomes of Split Learning, the first observation we can make is that matching performance drops, in terms of Precision, as the matching dataset size increases. However, we may extract some additional useful conclusions. First of all, we may see that both split classifiers, `-1-' and `-2-' exhibit similar performance considering the same kernel and Training dataset size. Next, it is easy to discern that, in terms of Precision, larger Training set sizes (dotted lines) exhibit significantly better performance than the cases where the 500 records training set had been employed. This difference is significant, reaching 0.15 of Precision, for the case of the 10000 matching records. On the other hand, compared to the case of Plain models, using large Training sets may deteriorate performance only by 5\%, which is the price to pay for achieving privacy. Finally, using smaller Training datasets causes a more significant drop in performance, illustrated by a steepest slope in Fig. \ref{fig:training_size_Precision}, as the size of the matching dataset rises. 

Let us now examine what happens in terms of Recall, as illustrated in Fig. \ref{fig:training_size_Recall}. Starting with the Plain SVM cases again, they achieve absolute Recall, no matter what kernel is used. Now, moving to the cases of Split Learning, the results are quite interesting, especially when considered in conjunction of those of Fig. \ref{fig:training_size_Precision}. To begin with, we may discern that Recall is not affected by the size of data to be matched, regardless  the Training set size or the kernel used for training. Nevertheless, using smaller Training sets, designated by solid lines, results in higher Recall, approximately 0.996, compared to the cases of using the 2000 records dataset for training. However, in the latter case recall is between 0.98 and 0.99. This means a less than 2\% drop compared to the ideal case. Considering, now, the results for Precision as well, it is evident that using larger Training sets results in high Precision at a very small cost of Recall, being a fair trade-off. To sum up, we have illustrated that at an expense of 5\% in Precision and less than 2\% in Recall, we have managed to provide privacy.


%For Precision, and considering the case of Linear Local SVM, we may discern that it exhibits the highest performance of all methods again, reaching 0.98, regardless of the Training Set size. The RBF Local SVM then follows when trained with the 2000 records dataset, exhibiting Precision between 0.96 and 0.975 , without being affected by the Dataset size to be matched. Its behavior is similar when the 500 records training dataset is used, but with lower performance, ranging between 0.93 and 0.96, without seeming to be affected by the matching Dataset size either. Moving to FedeM's implementations, we may deduce both for the Linear and the RBF SVMs that the training set size significantly affects their performance. With the 2000 records dataset, both methods reach the score of the local RBF SVM with a score near 0.95. Nevertheless, using a smaller training set, significantly affects the performance of both of these approaches, which is now also affected by the dataset size to be matched. Thus, achieving for the 10000 records dataset, Precision of 0.84 for the Linear SVM and 0.78 for the RBF SVM. Given these, we may conclude that increasing the training set size positively affects FedeM's Precision performance.

%For Recall, both local SVM implementations perform perfectly. For FedeM, its behavior is reversed compared to its Precision performance. For the 500 records Training set, both Linear and RBF SVMs achieve a score over 0.98. Increasing the Training set size, Precision drops for Linear to 0.95, while for RBF it drops to 0.90. This leads us to the conclusion that increasing the Training set size leads to a drop of Recall. In any case, however, the Linear kernel performs better. Thus, a good practice is to use a linear kernel, increasing the size of the training set, as in the privacy-preserving context precision is more important.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{media/times.eps}
    \caption{Matching times comparison.}
    \label{fig:matching times}
\end{figure}

\subsection{Evaluation of Time Performance}
Having seen how Split Learning-based Privacy-Preserving Matching behaves in terms of Precision and Recall, it would be interesting to see how much time these methods require to match data. First, of all, matching time is not affected by the size of the Reference Set used. To this end, we will report times for the cases we have used a Reference Set of 2000 records, with the cases of 200 records exhibiting minimal fluctuations. These results are illustrated in Fig. \ref{fig:matching times}, with the horizontal axis representing the size of the dataset to be matched, while the vertical one stands for time in seconds.

Starting with Linear SVMs, for each of the two parties 5.8 and 5.6 secs are required, on average, to match 2000 records, respectively. For 5000 records, these times are 17.8 and 16.6 secs, while for 10000 records, 58.8 secs elapsed in both cases. For the plain SVM, these times are 6,
9.3 and 21.4 secs. For the case of RBF SVMs, somewhat more time is required. To be more specific, for 2000 records, 7.6 and 7.3 secs elapsed at each party on average. For 5000 records, 28.8 and 27.7 secs were required and, finally, matching 10000 records requires 104.3 and 103.4 seconds on average. For the plain SVM classifier, these times are 7.5, 18 and 57 secs.


As we can see, although record linkage is, by nature, a problem requiring quadratic time when blocking techniques \cite{Chr12} are not employed (a fact that also holds for Privacy-Preserving Record Linkage), matching time scales do not scale quadratically, featuring only a minimal overhead when compared to the plain SVM classifier.



%The time require for our method to match records consists of Data Preparation time, Training Time and Testing Time. Data Preparation time is proportional to the sizes of the Reference Set and the size of the dataset to be matched. However, it is independent of the used kernel to be used. 


%To this end, for 200 reference rows, and for the three datasets, 6, 18 and 57 secs. are required, exhibiting a superlinear behavior. This is more evident with the 2000 reference rows. Then, approximately 28, 136 and 495 secs are respectively required. Training time requires for the Local Linear and RBF SVMs 16.4 and 17.7 secs on average for 500 training records and 19.8 and 22.5 for 2000 training records. For the Federated case these times are, as expected, elevated. For 500 records 19.6 and 19.8 secs are required for Linear and RBF training and 32.7 and 44.7 for 2000 records. Finally, Testing time is also affected, due to the increased representation of each feature vector. As such, while the Local Linear SVM may require for matching 6, 9 and 21 secs, FedeM requires 7, 19 and 57 secs respectively.
